PA-Boot: A Formally Verified Authentication Protocol for Multiprocessor Secure Boot

Hardware supply-chain attacks are raising significant security threats to the boot process of multiprocessor systems. This paper identifies a new, prevalent hardware supply-chain attack surface that can bypass multiprocessor secure boot due to the absence of processor-authentication mechanisms. To defend against such attacks, we present PA-Boot, the first formally verified processor-authentication protocol for secure boot in multiprocessor systems. PA-Boot is proved functionally correct and is guaranteed to detect multiple adversarial behaviors, e.g., processor replacements, man-in-the-middle attacks, and tampering with certificates. The fine-grained formalization of PA-Boot and its fully mechanized security proofs are carried out in the Isabelle/HOL theorem prover with 306 lemmas/theorems and ~7,100 LoC. Experiments on a proof-of-concept implementation indicate that PA-Boot can effectively identify boot-process attacks with a considerably minor overhead and thereby improve the security of multiprocessor systems.

==> macros.tex <==
\RequirePackage{todonotes}
% TODOS
%\setlength{\marginparwidth}{1.5cm}
\newcommand{\mccomment}[1]{\todo[color=blue!10,size=\small,fancyline,author=Mingshuai]{#1}\xspace}
\newcommand{\mccommentinline}[1]{\todo[inline,color=blue!10,author=Mingshuai]{#1}\xspace}
\newcommand{\atmc}{\colorbox{blue!10}{\textbf{@Mingshuai}}}

\newcommand{\zzcomment}[1]{\todo[color=green!10,size=\small,fancyline,author=Zhuoruo]{#1}\xspace}
\newcommand{\zzcommentinline}[1]{\todo[inline,color=green!10,author=Zhuoruo]{#1}\xspace}
\newcommand{\atzz}{\colorbox{green!10}{\textbf{@Zhuoruo}}}

\newcommand{\rccomment}[1]{\todo[color=cyan!30,size=\small,fancyline,author=Rui]{#1}\xspace}
\newcommand{\rccommentinline}[1]{\todo[inline,color=cyan!30,author=Rui]{#1}\xspace}
\newcommand{\atrc}{\colorbox{cyan!30}{\textbf{@Rui}}}

%check mark
\newcommand{\cmark}{\textcolor{ForestGreen}{\ding{51}}}%
\newcommand{\qmark}{\textcolor{Maroon}{\textbf{?}}}%

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=0.8pt,outer sep=8pt] (char) {#1};}}
\newcommand*\newcircled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=1.3pt,outer sep=3pt] (char) {#1};}}
%devil mark
\newcommand{\devil}{\begin{minipage}[c]{.75\baselineskip}\includegraphics[height=.75\baselineskip]{image/devil.png}\end{minipage}}

%event marks
\newcommand{\eventp}{\begin{minipage}[c]{1\baselineskip}\includegraphics[height=1\baselineskip]{image/event-p.pdf}\end{minipage}}
\newcommand{\eventq}{\begin{minipage}[c]{1\baselineskip}\includegraphics[height=1\baselineskip]{image/event-q.pdf}\end{minipage}}

%strikingthrough in red
\newcommand\redsout{\bgroup\markoverwith{\textcolor{red}{\rule[0.4ex]{2pt}{1.5pt}}}\ULon} 

%et al.
\newcommand{\etal}{\textit{et al}}

%colors
\definecolor{figyellow}{RGB}{255,242,204}
\definecolor{figyellow2}{RGB}{241,202,23}
\definecolor{figblue}{RGB}{218,232,252}
\definecolor{figgreen}{RGB}{213,232,212}

\definecolor{figgrey}{RGB}{175,171,171}
\definecolor{figgrey2}{RGB}{118,113,113}
\definecolor{figred}{RGB}{225,59,67}

\definecolor{OriginalProcess}{HTML}{D7191C}
\definecolor{ChallResp}{HTML}{FDAE61}
\definecolor{SesskeyGen}{HTML}{ABDDA4}
\definecolor{CertsValid}{HTML}{2B83BA}

\font\tt=rm-lmtl10
\font\btt=rm-lmtk10
%\newcommand{\code}[1]{{\fontfamily{cmtt}\fontseries{m}\fontshape{n}\selectfont\small{#1}}}
\newcommand{\code}[1]{{\fontfamily{cmtt}\fontseries{m}\fontshape{n}\selectfont#1}}
%\newcommand{\codeBold}[1]{{\ttfamily\fontseries{b}\fontshape{n}\selectfont#1}}
\newcommand{\codeBold}[1]{#1}
\newcommand{\system}{\code{PA-Boot}}
\newcommand{\systemBold}{\codeBold{PA-Boot}}
\newcommand{\csystem}{\code{CPA-Boot}}
\newcommand{\csystemBold}{\codeBold{CPA-Boot}}

%math symbols
\newcommand{\bools}{\ensuremath{\mathbb{B}}\xspace}
\newcommand{\TRUE}{\ensuremath{\mathtt{true}}}
\newcommand{\FALSE}{\ensuremath{\mathtt{false}}}
% \newcommand{\mathbcal}[1]{\mathcal{#1}}
\newcommand{\spec}{\ensuremath{\mathcal{S}}}
\newcommand{\prop}{\ensuremath{\mathcal{A}}}

\newcommand{\defeq}{{}\triangleq{}}
\newcommand{\ddefeq}{\ {}\defeq{}\ }
\newcommand{\eeq}{~{}={}~}
\newcommand{\wwedge}{~{}\wedge{}~}

%protocol functions
\newcommand{\hash}[1]{\ensuremath{\mathtt{Hash}\left(#1\right)}}
\newcommand{\verifycert}[2]{\ensuremath{\mathtt{validCert}\left(#1,#2\right)}}

%protocol symbols
\newcommand{\csr}{\ensuremath{\textit{CSR}}}
\newcommand{\cert}[1]{\ensuremath{\textit{Cert}_{\textit{#1}}}}
\newcommand{\pubk}[1]{\ensuremath{\textit{PubK}_{\textit{#1}}}}
\newcommand{\privk}[1]{\ensuremath{\textit{PrivK}_{\textit{#1}}}}
\newcommand{\epubk}[1]{\ensuremath{\textit{EPubK}_{\textit{#1}}}}
\newcommand{\eprivk}[1]{\ensuremath{\textit{EPrivK}_{\textit{#1}}}}
\newcommand{\nonce}[1]{\ensuremath{\mathcal{N}_{\textit{#1}}}}

\newcommand{\certroot}{\ensuremath{\cert{root}}}
\newcommand{\certbsp}{\ensuremath{\cert{BSP}}}
\newcommand{\certap}{\ensuremath{\cert{AP}}}
\newcommand{\pubkbsp}{\ensuremath{\pubk{BSP}}}
\newcommand{\pubkap}{\ensuremath{\pubk{AP}}}
\newcommand{\privkbsp}{\ensuremath{\privk{BSP}}}
\newcommand{\privkap}{\ensuremath{\privk{AP}}}
\newcommand{\privkroot}{\ensuremath{\privk{RT}}}
\newcommand{\epubkbsp}{\ensuremath{\epubk{BSP}}}
\newcommand{\epubkap}{\ensuremath{\epubk{AP}}}
\newcommand{\eprivkbsp}{\ensuremath{\eprivk{BSP}}}
\newcommand{\eprivkap}{\ensuremath{\eprivk{AP}}}
\newcommand{\noncecha}{\ensuremath{\nonce{AP}}}
\newcommand{\nonceresp}{\ensuremath{\nonce{BSP}}}
\newcommand{\sessk}{\ensuremath{\mathcal{K}_{\textit{s}}}}

\newcommand{\kpairbsp}{\ensuremath{\left\langle\pubkbsp,\privkbsp\right\rangle}}
\newcommand{\kpairap}{\ensuremath{\left\langle\pubkap,\privkap\right\rangle}}
\newcommand{\ekpairbsp}{\ensuremath{\left\langle\epubkbsp,\eprivkbsp\right\rangle}}
\newcommand{\ekpairap}{\ensuremath{\left\langle\epubkap,\eprivkap\right\rangle}}

\newcommand{\hashrc}{\ensuremath{\textit{RootCertHash}}}

%%protocol specifications
\newcommand{\states}{\ensuremath{S}\xspace}
\newcommand{\sink}{{\downarrow}}
\newcommand{\stable}{{\ensuremath{S^\sink}\xspace}}
\newcommand{\inistate}{\ensuremath{s_0}\xspace}
\newcommand{\idlstate}{\ensuremath{\bar{s}}\xspace}
\newcommand{\labels}{\ensuremath{\Lambda}\xspace}
\newcommand{\labseq}{\ensuremath{\Lambda\!^*}\xspace}
\newcommand{\trans}{\ensuremath{\Delta}\xspace}
\newcommand{\tran}{\ensuremath{\delta}\xspace}
\newcommand{\step}[3]{\ensuremath{#1 \xrightarrow{#2} #3}\xspace}
% \newcommand{\steps}[3]{\ensuremath{#1 \xhookrightarrow{{\raisebox{-2pt}{$ #2$}}} #3}\xspace}
\newcommand{\steps}[3]{\ensuremath{#1 \xhookrightarrow{\ThisStyle{\raisebox{-2pt}{$\SavedStyle #2$}}} #3}\xspace}
\newcommand{\run}{\ensuremath{\pi}\xspace}
\newcommand{\runs}{\ensuremath{\Pi}\xspace}

%utility functions
\newcommand{\tail}[1]{\ensuremath{\mathtt{Tail}\left(#1\right)}}
\newcommand{\configs}{\ensuremath{C}\xspace}
\newcommand{\context}{\ensuremath{\Gamma}\xspace}
\newcommand{\benign}{\ensuremath{\mathcal{B}}\xspace}
\newcommand{\mitm}{\ensuremath{\mathcal{M}}\xspace}

%formal symbols
\newcommand{\mydot}{\text{{\large\textbf{.}}\,}}

\newcommand{\init}{\ensuremath{\mathsf{INIT}}}
\newcommand{\error}{\ensuremath{\mathsf{ERROR}}}
\newcommand{\attacked}{\ensuremath{\mathsf{ATTACKED}}}
\newcommand{\abnormal}{\ensuremath{\mathsf{ABNORMAL}}}
\newcommand{\terminate}{\ensuremath{\mathsf{END}}}
\newcommand{\ok}{\ensuremath{\mathsf{OK}}}

\newcommand{\fpro}{\ensuremath{\mathsf{Processor}}}
\newcommand{\fbsp}{\ensuremath{\mathsf{bsp\_chip}}}
\newcommand{\fap}{\ensuremath{\mathsf{ap\_chip}}}
\newcommand{\fenv}{\ensuremath{\mathsf{env}}}
\newcommand{\fst}{\ensuremath{\mathsf{status}}}
\newcommand{\fprivk}{\ensuremath{\mathsf{private\_key}}}
\newcommand{\flnonce}{\ensuremath{\mathsf{local\_nonce}}}
\newcommand{\flsk}{\ensuremath{\mathsf{local\_share\_key}}}
\newcommand{\fsessk}{\ensuremath{\mathsf{session\_key}}}
\newcommand{\fcertroot}{\ensuremath{\mathsf{ca\_hash}}}
\newcommand{\fcb}{\ensuremath{\mathsf{certs\_buffer}}}
\newcommand{\fpb}{\ensuremath{\mathsf{packet\_buffer}}}
\newcommand{\frnonce}{\ensuremath{\mathsf{remote\_nonce}}}
\newcommand{\frsk}{\ensuremath{\mathsf{remote\_share\_key}}}

\newcommand{\levent}{\ensuremath{\mathtt{event\_enabled}}}
\newcommand{\lexec}{\ensuremath{\mathtt{exec\_op}}}
\newcommand{\lrun}{\ensuremath{\mathtt{run}}}
\newcommand{\lreach}{\ensuremath{\mathtt{reachable}}}
\newcommand{\lisatt}{\ensuremath{\mathtt{is\_attack}}}

%% Isabelle code
\newcommand{\isakey}[1]{\ensuremath{\textcolor{NavyBlue}{\textbf{#1}}}}
\newcommand{\record}{\isakey{record}}
\newcommand{\datatype}{\isakey{datatype}}
\newcommand{\defn}{\isakey{definition}}
\newcommand{\fun}{\isakey{fun}}
\newcommand{\field}[1]{\ensuremath{\mathtt{#1}}}
\newcommand{\type}[1]{\ensuremath{\textit{#1}}}

% RQ
%\newcommand{\rq}{\ensuremath{\mathcal{RQ}}}
\newcommand{\rques}[1]{\ensuremath{\mathbf{RQ}{\mathbf{#1}}}}

\newcommand{\flag}[1]{\ensuremath{\textnormal{#1}}}
\newcommand{\func}[1]{\ensuremath{\mathtt{#1}}}
\newcommand{\acronym}[1]{\ensuremath{\mathtt{#1}}}

\newcolumntype{?}{!{\vrule width 0.8pt}}

%%Environments styles
\theoremstyle{plain}
\newtheorem*{thm*}{Theorem}
\newtheorem*{exmp*}{Example}
\newtheorem*{counterexmp*}{Counterexample}

\newtheoremstyle{ourstyle}{}{}{\itshape}{}{\bfseries}{.}{ }{\thmname{#1}\thmnumber{ #2}\thmnote{ (#3)}}
%\newtheoremstyle{ourstyle}{}{}{}{}{\bfseries}{.}{ }{\thmname{#1}\thmnumber{ #2}\thmnote{ (#3)}}
\theoremstyle{ourstyle}

\newcounter{ctdef}
\newcounter{ctlem}
\newcounter{ctprop}

\newtheorem{theorem}{Theorem}
\newtheorem{definition}[ctdef]{Definition}
\newtheorem{lemma}[ctlem]{Lemma}
\newtheorem{property}[ctprop]{Property}
\newtheorem{corollary}[theorem]{Corollary}

%low-level lemma environment
\newtheoremstyle{llemstyle}{}{}{\itshape}{}{\bfseries}{.}{ }{\thmname{#1}~\thmnumber{\thectprop.#2}\thmnote{ (#3)}}
%\newtheoremstyle{ourstyle}{}{}{}{}{\bfseries}{.}{ }{\thmname{#1}\thmnumber{ #2}\thmnote{ (#3)}}
\theoremstyle{llemstyle}

\newcounter{ctllem}
\newtheorem{llemma}[ctllem]{Lemma}

%\newtheorem*{problem_formu}{Problem Formulation}
%\newenvironment{problem_formulation}
%{\begin{mdframed}\begin{problem_formu}}
		%		{\end{problem_formu}\end{mdframed}}

\newtheoremstyle{exmpstyle}{}{}{}{}{\bfseries}{.}{ }{\thmname{#1}\thmnumber{ #2}\thmnote{ (#3)}}
\theoremstyle{exmpstyle}

\newtheorem{example}[theorem]{Example}
\newtheorem{counterexample}[theorem]{Counterexample}

\newtheoremstyle{rmkstyle}{}{}{}{}{\bfseries}{.}{ }{\thmname{#1}\thmnote{ (#3)}}
\theoremstyle{rmkstyle}

%\newtheorem{remark}[theorem]{Remark}
\newtheorem{remark}{Remark}
%for qedT mark compatible within displaymath
\def\triangleforqed{\hbox{$\lhd$}}
\makeatletter
\DeclareRobustCommand{\qedT}{%
	\ifmmode
	\eqno \def\@badmath{$$}%$$
	\let\eqno\relax \let\leqno\relax \let\veqno\relax
	\hbox{\triangleforqed}%
	\else
	\leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
	\quad\hbox{\triangleforqed}%
	\fi
}
\makeatother
